SciCapenter: Supporting Caption Composition for Scientific Figures with Machine-Generated Captions and Ratings

Crafting effective captions for figures is important. Readers heavily depend on these captions to grasp the figure's message. However, despite a well-developed set of AI technologies for figures and captions, these have rarely been tested for usefulness in aiding caption writing. This paper introduces SciCapenter, an interactive system that puts together cutting-edge AI technologies for scientific figure captions to aid caption composition. SciCapenter generates a variety of captions for each figure in a scholarly article, providing scores and a comprehensive checklist to assess caption quality across multiple critical aspects, such as helpfulness, OCR mention, key takeaways, and visual properties reference. Users can directly edit captions in SciCapenter, resubmit for revised evaluations, and iteratively refine them. A user study with Ph.D. students indicates that SciCapenter significantly lowers the cognitive load of caption writing. Participants' feedback further offers valuable design insights for future systems aiming to enhance caption writing.

==> Sections/qualitative-result.tex <==
\paragraph{Preference for Caption Length} 

% template and concrete suggestions
\textit{P9 - So basically you want like, not only the check table, but also give you a suggestion what to write for the aspects. Just like the explanation part, maybe you can give me some suggestion about how to improve my caption. Because sometimes I saw the check table but I don't know how to use this check table to improve my caption. ... just high level sentences so for example you need to add something add something or it's better to explain something in the caption that's it.}

\textit{P10 -  maybe you can provide some suggestions, like just give a user, like what's, like after the explanation, just give an example of how to improve that. Then, like maybe for each point, you can list a sentence or two sentences, like that can be added to caption directly or user can modify like reference to the recommendation and add to the system. So user don't need to come up by themselves. So the points, each point, you mean the check table? Yeah, like the check table, like, so yeah, because for instance, if the stats are missing, so basically, the explanation only tells you that it's missing, you should add it. So what I mean is, so our system should also provide an example of what can be added, like something like that. So that might be more helpful for users to add the caption.}


\textit{P11 - Maybe you can just give me a roughly paragraph to guide me how to describe this figure. And you can tell me what kind of result and what kind of the highlight point I need to mention. You can give me a hint, so that like the bullet point, so that I can, when I do my paper, I can just follow the guidelines of the systems to finish all the writing of the paragraph. Okay. So basically you want some, like standard structure. Just a structure, not the exact for the paragraph that you need to mention like a curve is higher than b curve at which point so you need to tell me, remind me that which point should i point out in my paper}

\textit{P13 - let's say for the caption, I typed X, Y Z based on the recommendations that you had given. And I wanted one more offer recommendation that says how I can make XYZ that better. instead of long, short, and paragraph, I wanted one more that says, okay, the input that you gave, how can I make that itself better? Based on  the check table, you're like, Oh, I know that. There is a paragraph explaining how I can make it better. But I would also like to see an answer as well, if that makes sense. basically, you want to like refine for the specific aspect? Yes, exactly. if something like GPT-4, you could give my caption as well as the explanation combined to generate a better caption. And I would be like, Oh, I can definitely use those guidelines as well. Because I think the explanation was too big and wasn't in the mood to read the whole thing.
}

% different opinion of same feature
\textit{P3 - I think with your system, the good side about it is it has a check table, so it kind of reminds me, you know, which element I should put or which criteria I should be checking before I write the caption or while I'm writing the caption. Whereas when I was in Task1 and Task2, I really don't know. I'm a little bit lost. I didn't really know how to put and what kind of things I should be mindful when I'm writing my caption.}

\textit{P4 - I do think that the check table and also it's really helpful because I can know what information is missing in my caption}

\textit{P5 - it was organized in a very clear way for me to understand which part I need to improve. Like, whether I delivered a clear message of the figure how I could improve how I could add more stats, I could add more stats into the caption. And also whether the caption is clear enough for the reader. So I think the comments after I submit and also the check table is really helpful for me to improve the caption .
}

\textit{P9 - Because I saw this check table but I don't know how to use this check table to to improve my caption because it sometimes says you need to add stats for the caption, but for the figure, actually I'm not able to add some statics for these figures}

\textit{P11 - And for the checkbox. I think some of the features is not I really want to have in my caption. So let's maybe just three or two of them I want to put in my caption. So sometimes I don't mind whether it is in the checkbox or not.}

\textit{P12 -  I don't like that I don't check every part of it because I think in some cases you don't need to cover all the things, just one sentence which is enough.}


\begin{itemize}
    \item Short Captions: Most participants (e.g., P1, P4, P7, P10, P11, P14) prefer short captions, emphasizing conciseness and simplicity. They typically mention only the purpose of the plot or critical points.
    \item Long Captions: Few others (e.g., P3, P13) favor long captions for their informativeness, especially when the figure is complex or significant.
\end{itemize}

\paragraph{Preferred Content of Captions}


\begin{itemize}
    \item Most agree that captions should avoid repeating information detailed in the main text, instead offering a summary or highlighting key points (P3, P7, P11, P15).
    \item Captions should be self-contained to some extent, giving readers a clear idea of the figure without needing to refer back to the text (P8).
\end{itemize}

\paragraph{Usefulness of System Features}


\begin{itemize}
    \item Check Table: The check table's effectiveness varies. Some find it confusing or irrelevant to their needs (P9, P11, P12), while others appreciate its guidance on what to include in a caption (P3, P4, P5, P7, P15).
    \item Paragraphs \& Explanations: The provided paragraphs and explanations are generally seen as helpful for understanding and describing figures (P2, P3, P6, P15), but sometimes explanations have certain template not actually capture the modification (P4, P8) and paragraph miss catching some contents (P5).
    \item Generated Captions: The system-generated captions often fall short of expectations, with some experiencing inaccuracies or "hallucinations" (P8, P10, P11, P15), especially short captions.

    \textit{P8 -  I think the generation wasn't 100\% precise. Of course not, but like, sometimes it captures some weird stuff. But it's also nice that some keywords could also be used, like just describe when you're writing}

    \textit{P10 - the long and short caption, I think maybe because of our reason or something, it wasn't that good}

    \textit{P11 - for the long captions, I don't think it's useful because for my personal preference I don't like the long captions, but for the short captions, sometimes it doesn't meet my requirement}

    \textit{P15 - So for the generated caption, why is not useful? Because it just have some hallucination, or they just write what you don't want? Sometimes it had some hallucinations and sometimes they were not useful. I don't think they are explaining to figure well.}
\end{itemize}

\paragraph{Suggestions for Improvement}

\begin{itemize}
    \item Some participants suggest generating caption template for similar domain or figures would be helpful (P7, P8, P11) 
    
    \textit{P7 - If you can generate a typical caption from other people that have already published ..., like, you have standard and you just need to fill the detailed,}
    
    \textit{P8 - I would be curious about how other people do for similar figures. ..., I would like to see how people mention in similar domain of papers for similar format of the figure.}
    
    ,others suggest more personalized or different style recommendation for long/short captions (P2, P4, P5, P15). 
    % \item The idea of having a feature to assist with overall paper structure and coherence is also popular (P14).
    \item Some desire more interaction with the system in refining captions (P4, P5, P12).
\end{itemize}

\paragraph{System Reliability and Feedback}

\begin{itemize}
    \item There is a mixed response to the system's scoring and feedback. Some find it reassuring and useful (P2, P4, P15), while others question its accuracy or relevance (P1, P3, P6).
    \item The need for more precise and constructive feedback is a common request.
\end{itemize}
